AQD: Towards Accurate Fully-Quantized Object Detection

Network quantization allows inference to be conducted using low-precision arithmetic for improved inference efficiency of deep neural networks on edge devices. However, designing aggressively low-bit (e.g., 2-bit) quantization schemes on complex tasks, such as object detection, still remains challenging in terms of severe performance degradation and unverifiable efficiency on common hardware. In this paper, we propose an Accurate Quantized object Detection solution, termed AQD, to fully get rid of floating-point computation. To this end, we target using fixed-point operations in all kinds of layers, including the convolutional layers, normalization layers, and skip connections, allowing the inference to be executed using integer-only arithmetic. To demonstrate the improved latency-vs-accuracy trade-off, we apply the proposed methods on RetinaNet and FCOS. In particular, experimental results on MS-COCO dataset show that our AQD achieves comparable or even better performance compared with the full-precision counterpart under extremely low-bit schemes, which is of great practical value. Source code and models are available at: https://github.com/ziplab/QTool

==> method-backup.tex <==

\section{Proposed method}
\subsection{Preliminary} 

\subsubsection{Quantized value representation
}
\label{sec:representation}


Full-precision (32-bit) floating-point is a general data type that is used in representing data in deep learning models. With network quantization, the continuous full-precision %
weights and activations are discretized to limited number of quantized values. Specifically, given a specific bitwidth $b$, the total number of quantized values is $2^b$. To enable efficient integer arithmetic operations on the quantized values, it requires that the quantization scheme be a mapping of real values to integers.
Formally, for $b$-bit quantization of any full-precision value $r \in \mathbf{R}$,
its quantized version $\overline{r}$ 
can be formulated as:
\begin{equation}
\label{eq:represnet-linear}
\overline{r} = \eta \cdot \alpha,
\end{equation}
where $\alpha$ is a full-precision floating-point scale factor shared for the whole tensor $\bf{R}$, and $\eta \in {\mathbb{N}}$ implies the corresponding mapping value in the integer domain.


\subsubsection{Quantization function}
\label{sec:function}
In this work, we propose to quantize both weights and activations with learnable quantization intervals motivated by LSQ~\cite{Esser2020LEARNED}.
Without loss of generality, given a convolutional layer or fully-connected layer in a network, the weight $\mathbf{W}$ is convolved with the input activation $\mathbf{X}$, where $\bw$ and $\bx$ are real-valued tensors.
We use $x, w \in \mathbb{R}$ to denote the element of $\bX$ and $\bW$ respectively. 
Let $\nu_x$ and $\nu_w$ be the trainable quantization interval parameters that indicate the range of activations and weights to be quantized.

For a given $x$, we first constrain it to the range $[0, \nu_x]$, with values out of the range clipped into boundaries. We then linearly map values in interval $[0, \nu_x]$ to the integer domain of ${0,1,\hdots, 2^b-1}$, where $b$ is the quantization bitwidth. At last, we restore the magnitude of the original $x$ by multiplying the corresponding scale factor. Formally, the quantization process can be formulated as follows:
\begin{equation}
\label{eq:mapping-fm}
\begin{aligned}
&\eta_x  = \lfloor {\rm clip} (\frac{x}{\nu_x}, 0, 1) \cdot (2^b -1) \rceil, \\
&  \overline{x} =  \eta_x \cdot \frac{\nu_x}{2^b-1},
\end{aligned}
\end{equation}
where $\lfloor \cdot \rceil$ returns the nearest integer of a given value, $\mathrm{clip}\left(x, x_\mathrm{low}, x_\mathrm{up}\right) = {\rm min}({\rm max}(x,x_\mathrm{low}),x_\mathrm{up})$, 
$\eta_x$ is the corresponding integer-domain mapping value of $x$, and $\frac{\nu_x}{2^b-1}$ is the magnitude-restore scale factor. 

For given $w$ from weight parameters, the quantization interval is defined as $[-\nu_w, \nu_w]$.
We compute the quantized value $Q_W(w)$ similar to $Q_X(x)$ except that an additional transformation is applied 
, which can be formulated as:
\begin{equation}
\label{eq:mapping-wt}
\begin{aligned}
&\eta_w = \lfloor ({\rm clip} (\frac{w}{\nu_w}, -1, 1) + 1) /2 \cdot (2^b -1) \rceil, \\
    & \overline{w} = (\eta_w \cdot \frac{1}{2^b-1} \cdot 2 -1) \cdot \nu_w, 
\end{aligned}
\end{equation}
where $\eta_w$ is the corresponding integer-domain mapping value of $w$. 

During network training, the discretization operation by $\rm rounding$ function $\lfloor \cdot \rceil$ is non-differentiable. To avoid gradient vanishing issue, we employ the Straight-Through Estimator (STE) for back-propagation \cite{bengio2013estimating}.


\subsection{Floating-point Free Quantization}
In this paper, we present an Accurate Quantized object Detection (AQD) method that fully gets rid of floating-point computation while still achieving promising performance. 
In a conventional residual block as shown in Figure \ref{fig:quant-flow}, we propose to substitute floating-point operations for fixed-point operations 
in all kinds of layers, including the convolutional layer, batch normalization layer and skip connections. In this way, only integer arithmetic is required during network inference, which greatly reduces the computational overhead of the network. In the following subsections, we will introduce the details of the proposed method regarding fixed-point operations for each of these layers.


\begin{figure}[!t] 
    \centering
	\includegraphics[width=0.9\linewidth]{figures/quant-flow.pdf}
	\caption{xxx} 
	\label{fig:quant-flow} 
\end{figure}

\subsubsection{Convolutional and Fully-connected Layers}
\label{sec:conv}

As mentioned in Section~\ref{sec:representation},  we define a unified tensor representation, and all tensors in the quantized network are required to follow the rule 
in Eq. (\ref{eq:represnet-linear}).
In this subsection, we %
explicitly demonstrate that the quantization scheme presented in Section \ref{sec:function} is also compatible with the representation format for input activations, weights as well as the output activations.



Note that the quantization interval parameters $\nu_x$ and $\nu_w$ are shared for all elements in $\bX$ and $\bW$, respectively. Therefore, the output activation of a quantized convolutional or fully-connected layer can be written as: 
\begin{equation}
\label{eq:mapping-conv}
\begin{aligned}
\overline{x} \cdot \overline{w} &= (\eta_x \cdot \frac{\nu_x}{2^b-1}) \cdot ((\eta_w \cdot \frac{1}{2^b-1} \cdot 2 -1) \cdot \nu_w) \\
 & = (\eta_x \cdot (2 \cdot \eta_w - 2^b + 1)) \cdot \frac{\nu_x \cdot \nu_w}{(2^b-1)^2}, \\
 & = \eta_{\rm{conv}} \cdot \alpha_{\rm{conv}}.
\end{aligned}
\end{equation}
Benefit from the data representation in Eq. (\ref{eq:represnet-linear}), the scale factor of $x$ and $w$ can be handled independently from $\eta_x$ and $\eta_w$. We can easily observe that the output activation also fits the uniform quantization format in Eq. (\ref{eq:represnet-linear}). The bitwidth of the output value is expected to be larger than $2\cdot b$ with the maximum value being determined by the network configuration (\eg, convolutional kernel size and channel number).
Note that the floating-point scale factor $\alpha_{\rm conv}$
can be passed to the proceeding layer directly. In this case, only fixed-point operations exist in the quantized convolutional or fully-connected layer, which can greatly reduce the computational cost.

\subsubsection{Normalization Layers}
\label{sec:normalization}

\begin{figure*}[!t] 
	\centering
	
	\subfigure[1-th layer of classification head]{ 
		\label{fig:first_layer_cls_head} 
		\includegraphics[height=1.18in]{figures/dist_cls_norm0.pdf}
		} 
	\subfigure[1-th layer of regression head]{ 
		\label{fig:first_layer_reg_head} 
		\includegraphics[height=1.18in]{figures/dist_bbox_norm0.pdf}
		} 
	\subfigure[2-th layer of classification head]{ 
		\label{fig:second_layer_cls_head}  
		\includegraphics[height=1.18in]{figures/dist_cls_norm1.pdf}
		} 
	\subfigure[2-th layer of regression head]{ 
		\label{fig:second_layer_reg_head} 
		\includegraphics[height=1.18in]{figures/dist_bbox_norm1.pdf}
		} 
	\caption{\bohan{replace the 1-th layer with other layers. Also is it distribution of batch statistics or feature maps?}Distribution of batch statistics at the batch normalization layer of a 2-bit ResNet-18 FCOS detector. Level-x denotes that the prediction are made on the x-th pyramid level. Different pyramid levels of feature show different batch statistics.} 
	\label{fig:histograms_batch_statistics} 
\end{figure*}

Both batch normalization (BN)~\cite{ioffe2015batch}
and group normalization (GN)~\cite{wu2018group} are widely used in classical object detection networks, such as RetinaNet \cite{lin2017focal} and FCOS \cite{tian2019fcos}. We investigate the differences of these two normalization operators and analyze their impact on the network quantization and inference. 

In particular, BN is employed mainly in the backbone module for feature extraction. In contrast, GN is preferred in the detection head part, as the head is generally shared to handle extracted feature of different levels in the feature pyramid network (FPN) \cite{lin2017feature}. Both BN and GN normalize the input activations using means and variance with an optional affine transformation. However, these two normalization strategies differ in two aspects.
On the one hand, a BN layer calculates the statistics of the whole mini-batch while those of the group normalization only reply on the individual input tensor in the mini-batch. Thus, BN is more sensitive to the training batch size, and might suffer from inaccurate statistics when the batch size is small. In contrast, GN behaves more stable to the training batch size.
On the other hand, BN keeps track of exponential moving average mean $\mu$ and variance $\sigma$, and update them using the minibatch statistics at each forward step during training, while $\mu$ and $\sigma$ are \textbf{fixed} during inference. 
In contrast, GN \textbf{re-computes} the statistics information in each forward step during both training and inference procedures. As a result, GN unavoidably incurs floating-point computation during inference. Moreover, compared with BN, which can be potentially fused into the corresponding convolutional layer with no extra computational cost, GN imposes more execution burden during inference. 

To allow for integer-only arithmetic, we suggest to use batch normalization to replace group normalization in quantized detection networks.
The replacement might introduce training instability to the detectors, as a small training batch size is commonly used. %
Fortunately, when equipped with the synchronized version of batch normalization (Sync-BN), the inaccurate statistics issue of batch normalization can be largely relieved \cite{peng2018megdet}.
However, another issue may occur when FPN \cite{lin2017feature} is employed in the detectors, where
a large divergence of batch statistics between different feature pyramid levels is observed, as shown in Figure~\ref{fig:histograms_batch_statistics}.
Therefore, using shared BN statistics across prediction heads may lead to highly degraded estimates of statistical quantities, which will cause a significant performance drop. 
To solve this issue, we propose 
multi-level batch normalization (multi-level BN) to attain better quantization performance. Specifically, multi-level BN privatizes batch normalization layers for the shared convolutional layer in different detector heads. 
The proposed multi-level BN can capture individual batch statistics of the corresponding feature level. Furthermore, only negligible parameters (less than 1.1\% of the model size) are introduced. Besides, it should be noted that only one batch normalization is activated at the same time though multiple batch normalization are allocated (as extracted features from different levels are computed sequentially). Thus, the presented multi-level BN will not increase the computational cost compared with traditional shared batch normalization (or group normalization). 


\begin{figure}[!t] 
    \centering
	\includegraphics[width=0.9\linewidth]{figures/Multi-Level-BN.pdf}
	\caption{Illustration of the proposed quantized detection heads design. (a) Conventional detection frameworks with shared group normalization or batch normalization \cite{tian2019fcos,lin2017focal}; (b) The proposed multi-level BN that privatizes batch normalization layers for different heads.} 
	\label{fig:multi-level-BN} 
\end{figure}

 
In terms of efficiency, as floating-point operations exist in the batch normalization layer, we now design the corresponding quantization strategy to enable integer-only computation. 
We assume the previous layer is a quantized convolutional or fully-connected layer, whose output is $\overline{x} \cdot \overline{w}$ as explained in Eq. (\ref{eq:mapping-conv}).
Batch normalization layer then takes it as input and obtain the normalized result $z$.
Before quantizing the batch normalization layer, the normalized value $z$ can be computed by  

\begin{equation}
\begin{aligned}
\label{eq:bn-3}
z &= \frac{\eta_{\rm{conv}} \cdot \alpha_{\rm{conv}} - \mu}{\sqrt{\sigma^2 + \epsilon}} \cdot \gamma + \beta, \\
 &= (\eta_{\rm{conv}} + \frac{\beta \cdot \frac{\sqrt{\sigma^2 + \epsilon}}{\gamma} - \mu}{\alpha_{\rm{conv}}}) \cdot \frac{\alpha_{\rm{conv}} \cdot \gamma}{\sqrt{\sigma^2 + \epsilon}}, \\
 &= (\eta_{\rm{conv}} + s) \cdot \alpha_z,
\end{aligned}
\end{equation}
where $\gamma$, $\beta$ are the affine transformation parameters, $\epsilon$ is a constant to stabilize the computation.
Then we are able to obtain the quantized batch normalization layer by quantizing $s$:
\begin{equation}
\overline{z} = (\eta_{\rm{conv}} + \lfloor s \rceil) \cdot \alpha_z = \eta_z \cdot \alpha_z 
\end{equation}
Thereby, for quantized batch normalization, the main computation is the $\rm add$ operation between $\eta_{\rm{conv}}$ and $\lfloor s \rceil$ with the floating-point factor $\alpha_z$ passed to next layer directly.

It is worth noting that, compared with the output of the quantized convolutional or fully-connected layer, the quantized output $\overline{z}$ of the batch normalization layer still meets 
the uniform integer-aware representation in Eq. \ref{eq:represnet-linear}, but with the channel-wise scale factor $\alpha_z$.


\subsubsection{Skip Connections}
\label{sec:skip_connection}
 
 Skip connections are commonly applied in ResNet backbone and the FPN tower. In this subsection, we talk about how to enable integer-only computation of the skip connection layer (\ie, $\rm add$ operation between two tensors). Diving into the structure of object detection network, we can learn that skip connection is employed mainly in three occasions: (1) fusing of identify-mapping input $x$ and batch normalization output $\overline{z}$ in residual block (as illustrated in Figure \ref{fig:quant-flow}), (2) fusing of batch normalization outputs of the down-sampling branch and main branch in residual block, (3) fusing of the up-scaled feature map and current level feature map in FPN. 
 For either of these occasions, given the two input quantized values $x_1$ and $x_2$, the output of skip connection $y$ and its quantized value $\overline{y}$ are computed as follows, %
 \begin{equation}
 \label{eq:skip-1}
 \begin{aligned}
 y &= x_1 + x_2 = \eta_{1} \cdot \alpha_{1} + \eta_{2} \cdot \alpha_{2}, \\
 \overline{y} &= \left\{
\begin{array}{ll}
(\eta_{1} + \eta_{2} \cdot F(\alpha_{2}, \alpha_{1}) ) \cdot \alpha_{1}  & {\rm{if}} \;  \alpha_{2} \geq \alpha_{1} \\
(\eta_{1} \cdot F(\alpha_1, \alpha_2) + \eta_{2} ) \cdot \alpha_2 & \rm{otherwise}
\end{array}
\right.,
 \end{aligned}
 \end{equation}
 where function $F(\cdot)$ is defined as
 
\begin{equation}
\label{eq:skip-3}
F(m, n) = \frac{c}{2^d}, {\rm where~c, d} = \argmin_{c \in \mathbb{N}, d \in \mathbb{N_+}} {| \frac{m}{n}  - \frac{c}{2^d}|}.
 \end{equation}

Function $F(\cdot)$ actually is used for searching an approximation of a given fraction $\frac{m}{n}$ (where $m \geq n$). The approximation consists of a numerator part $c$ and a denominator part $2^d$. In particular, the numerator part $c$ is constrained to be an integer and the denominator part $2^d$ is constrained to be a bit-shift ($d$ is a positive integer). Function $F(\cdot)$ finds the best combination of $c$ and $d$ to approximate $\frac{m}{n}$. There is limited choice for $d$, for example $d \in \{0, 1, 2, \hdots, 31\}$ if $\eta_1$ and $\eta_2$ are represented in $32$-bit integer.
Therefore, function $F(\cdot)$ can be quickly solved, and Eq. (\ref{eq:skip-1}) can be implemented with fixed-point operations only (the scale factors $\alpha_1$ and $\alpha_2$ do not participate in computation and just passed to the next layer directly). Note that, Eq. (\ref{eq:skip-1}) is conducted in channel-wise manner since the scale factor is calculated for each channel in the batch normalization layer. 

 \subsubsection{Other Layers}
 
 Layers such as max-pooling and nearest interpolation do not introduce floating-point computation. Besides, they do not change the scale factors of input. Thus, there is no special modifications for these layers.


\subsection{Discussion}

\bohan{2: must discuss with BN folding, e.g., in FQN}


Compared with FQN, our method gets rid of the floating-point operations in the batch normalization layer.

To handle the skip connection layer, FQN constrains the scale factors from the two input activations with strict condition:

\begin{equation}
\label{eq:discuss-1}
\frac{\alpha_1}{\alpha_2} = 2^d
 \end{equation}
 where $d$ is an integer (different with the scope in Eq. \ref{eq:skip-3}, $d$ here can be either positive or negative). The FQN's constraint is equivalent to Eq. \ref{eq:skip-3} if forcibly fixing $c$ in Eq. \ref{eq:skip-3} constantly to be 1. Differently, our methods do not have such constraints. Actually, the proposed method allows to quantize different branches or layers completely independently. Moreover, no special consideration needs to pay on the quantization algorithm design, only if the quantized value meets Eq. \ref{eq:represnet-linear}. Therefore, higher quantization performance can potentially be obtained.
 


==> method-old.tex <==

\section{Proposed method}
    In this section, we describe the proposed accurate quantized object detection (AQD). We first introduce the definition of the quantization function in Section~\ref{sec:problem_definition}. Then we introduce the two hardware-friendly quantization methods, \ie, multi-level batch normalization (multi-level BN) in Section~\ref{sec:multi_level_bn} and xxx in Section~\ref{}, respectively.

	\subsection{Quantization function revisited}
	\label{sec:problem_definition}
	We consider build a one-stage quantized detector for object detection. One-stage object detector consists of a backbone, a feature pyramid and prediction heads. For a convolutional layer in a detector, we define the input $\bX$ and weight parameter $\bW$. Let $x_m$ and $w_m$ be the $m$-th element of $\bX$ and $\bW$, respectively. Here, we omit the subscript $m$ for convenience. Quantization seeks to reduce the bitwidth of $w$ and $x$ via quantizers:
	\begin{equation}
	\label{eq:quantizer}
	\begin{split}
	Q_{\bW}: ~& {w \stackrel{T_{\bW}}{\longrightarrow} \hat{w} \stackrel{D_{\bW}}{\longrightarrow} \bar{w}} \\ 
	Q_{\bX}: ~& {x \stackrel{T_{\bX}}{\longrightarrow} \hat{x} \stackrel{D_{\bX}}{\longrightarrow} \bar{x}} ,
	\end{split}
	\end{equation}
	where a quantizer $Q_{\Delta}(\Delta \in\{ \bW, \bX \})$ contains a transformer $T_{\Delta}(\Delta \in\{ \bW, \bX \})$ and a discretizer $D_{\Delta}(\Delta \in\{ \bW, \bX \})$. Following~\cite{Esser2020LEARNED}, the transformer $T_{\Delta}(\Delta \in\{ \bW, \bX \})$ transforms the value $v$ to $\left[ -Q_N, Q_P \right]$ with learnable step size $s$. Let $k$ be the bitwidth of the weights and activations of the quantized networks. For weights, $Q_N$ and $Q_P$ are $2^{k-1}$ and $2^{k-1}-1$. For activations, $Q_N$ and $Q_P$ are $0$ and $2^{k}-1$. The discretizer $D_{\Delta}(\Delta \in\{ \bW, \bX \})$ maps the continuous value $\hat{v}$ in the range $\left[ -Q_N, Q_P\right]$ to some discrete value $\bar{v}$.
	
		During the training of the quantized network, the gradient of step size $\partial \mL/\partial s$ is defined as follow:
	\begin{equation}
	    \frac{\partial \mL}{\partial s} = \sum_{i} \frac{\partial \mL}{\partial \bar{v}_i} \frac{\partial \bar{v}_i}{\partial s},
	\end{equation}
	where $i$ is over all elements in the corresponding layer. The summation over all elements makes the gradient of step size $\partial \mL/\partial s$ much larger than the gradient of the input value $\partial \mL/\partial v$. Hence,  directly training the quantized network with learnable step size is unstable. One possible solution is to rescale the gradient~\cite{Esser2020LEARNED}. However, it is hard to determine the value of scaling factor. The improper gradient scaling factor may hamper the performance of the quantized network. 
	
	To solve this issue, we propose a learned interval quantization (LIQ) method to quantize the network with trainable interval instead of step size, which can avoid rescaling the gradient. The transformer and discretizer  for the proposed LIQ can be defined as follow:
	
	\textbf{Transformer}: The transformer $T_{\Delta}(\Delta \in\{ \bW, \bX \})$ transforms the weights and activations to $\left[ 0, 1 \right]$, which are defined as follows:
	
	\begin{align}
    \hat{w} = T_{\bW} (w) =& \frac{1}{2} \cdot ( \max(-1, \min(\frac{w}{\alpha_{\bW}}, 1)) + 1) \\
	\hat{x} = T_{\bX} (x) =& \max(0, \min(\frac{x}{\alpha_{\bX}}, 1)),
	\end{align}
	where $\alpha_{\bW}$ and $\alpha_{\bX}$ are trainable interval parameters that limits the range of weights and activations.
	
	\textbf{Discretizer}: The discretizer $D_{\Delta}(\Delta \in\{ \bW, \bX \})$ maps the continuous value $\hat{v}$ in the range $\left[ 0, 1\right]$ to some discrete value $\bar{v}$, which is defined as follow:
	\begin{align}
	\label{eq:discretizer_weight}
	\bar{v} = D_{\Delta} (\hat{v}) =&  \mathrm{round}(\hat{v} \cdot q) \cdot{\frac{1}{q}},
	\end{align}
	where $q$ is the number of discrete values (except 0). Let $k$ be the bitwidth of the weights and activations of the quantized networks. Then, $q$ can be computed as $q = 2^{k} - 1$. After weights and activations quantization, we use affine transformation to bring the range of weights to $[-\alpha_{\bW}, \alpha_{\bW}]$ and range of activations to $[0, \alpha_{\bX}]$.
	
	\textbf{Back-propagation with gradient approximation}: 
	In general, the discretizer function is non-differentiable. Therefore, it is impossible to train the quantized network through back-propagation. To solve this issue, we use the straight-through estimator~\cite{bengio2013estimating, courbariaux2016binarized, zhou2016dorefa} (STE) to approximate the gradients. Then, we can use following equations to compute the gradient of $\partial \bar{w}/\partial \alpha_{\bW}$ and $\partial \bar{x}/\partial \alpha_{\bX}$ respectively:
	\begin{equation}
    	\frac{\partial \bar{w}}{\partial \alpha_{\bW}}= \left\{\begin{array}{ll}
        \mathrm{round}(\frac{w}{\alpha_{\bW}})-\frac{w}{\alpha_{\bW}} & |w| <\alpha_{\Delta} \\
        1 & |w| \ge \alpha_{\Delta}
        \end{array}\right. ,
    \end{equation}
    
    \begin{equation}
    	\frac{\partial \bar{x}}{\partial \alpha_{\bX}}=\left\{\begin{array}{ll}
        \mathrm{round}(\frac{x}{\alpha_{\bX}})-\frac{x}{\alpha_{\bX}} & x <\alpha_{\Delta} \\
        1 & x \ge \alpha_{\Delta}
        \end{array}\right. .
    \end{equation}


    \subsection{Multi-level batch normalization}
    \label{sec:multi_level_bn}
    
    \bohan{Introduce previous methods use GN and BN. GN need full-precision operations, So we use BN to avoid it. Then add our descriptions.}
    During the training of the quantized detector, batch normalization~\cite{ioffe2015batch} normalize the input features and update exponential moving average (EMA) statistics $\mu_{EMA}$ and $\sigma_{EMA}$ with current batch statistics $\mu$ and $\sigma$. 
In one-stage object detection frameworks, each prediction head encodes a corresponding feature level. However, due to the quantization process, there may be large divergence of batch statistics between different feature levels, as shown in Figure~\ref{fig:histograms_batch_statistics}. Therefore, using a shared batch normalization across prediction heads may lead to inaccurate batch statistics, which will cause a significant performance drop. 
    
    To solve this issue, we propose a simple yet effective method, called multi-level batch normalization (multi-level BN), that uses independent batch normalization for different feature levels.
    The multi-level BN can capture individual batch statistics of the corresponding feature level. There are two advantages of our method comparing to the standard shared BN strategy. First, multi-level BN only introduces negligible parameters. 
    In fact, multi-level BN only has less than 1.1\% of the model size. Second, multi-level BN does not change the architecture of the network. Therefore, the proposed multi-level BN does not increase any additional computational cost. An empirical study on the effect of multi-level BN can be found in Section~\ref{sec:effect_multi_level_bn}.
  
    
    \subsection{xxx}
    \label{sec:fully_quantized}


